Improving Rare Word Recognition with LM-aware MWER Training

Language models (LMs) significantly improve the recognition accuracy of end-to-end (E2E) models on words rarely seen during training, when used in either the shallow fusion or the rescoring setups. In this work, we introduce LMs in the learning of hybrid autoregressive transducer (HAT) models in the discriminative training framework, to mitigate the training versus inference gap regarding the use of LMs. For the shallow fusion setup, we use LMs during both hypotheses generation and loss computation, and the LM-aware MWER-trained model achieves 10\% relative improvement over the model trained with standard MWER on voice search test sets containing rare words. For the rescoring setup, we learn a small neural module to generate per-token fusion weights in a data-dependent manner. This model achieves the same rescoring WER as regular MWER-trained model, but without the need for sweeping fusion weights.

==> 2_hat.tex <==
\section{Review of HAT}
\label{sec:method}
\vspace*{-0.5ex}

%Introduce that HAT is a variant of RNNT and explain the factorization and what is the gist of internal LMs.

\TS{weiran: instead of $P_{E2E}$ should we say $P_{e2e}$ in this and next section?}
\WW{Probably does not matter. Let us use E2E?}

In this section, we review the Hybrid Autoregressive Transducer (HAT), as first presented in \cite{variani2020neural}. HAT can be seen as a variant of RNN-T~\cite{Graves_12a} with a factorized output distribution over the vocabulary, conditioned on whether to emit a non-blank token at each frame. 

It has a internal LM for modeling the distribution over non-blank label sequences, whose scores can be computed by feeding zero acoustic features to the HAT decoder. The interal LM captures the bias from seeing limited text data during ASR training (with audio-text pairs), and replacing the internal LM with an external LM trained on large amount of text data effectively corrects this bias.

% This factorization is critical to combine scores from an E2E and language model. 

An E2E model directly estimates the posterior of word sequence, $Y$, conditioned on the acoustic features, $X$, i.e.,  $P_{\text{E2E}}(y|x)$. 

A common way to integrate an E2E model with an external LM that estimates $P_{\text{ELM}}(Y)$ is to perform shallow fusion (Eq \ref{eq:shallow_fusion}).

%, as shown in Equation~\ref{eq:shallow_fusion}:
\begin{equation}
\centering
Y^* = \arg \max_Y \left[\log P_{\text{E2E}}(Y|X) + \gamma \log P_{\text{ELM}}(Y)\right]
\label{eq:shallow_fusion}
\end{equation}
Here, $\gamma$ is the weight given to the external LM. Since E2E models tend to be over-confident in their posterior estimates, weighting the two terms becomes difficult and can often lead to high deletions \cite{Chorowski2017}.  To address this issue, Hybrid Autoregressive Transducer (HAT) proposes a way to factor out an internal LM score, $P_{\text{ILM}}(Y)$, so that the likelihood score from the E2E model, $P_{\text{E2E}}(X|Y)$, can be approximated by Equation \ref{eq:ilm}:
\begin{equation}
\centering
\log P_{\text{E2E}}(X|Y) \approx \log P_{\text{E2E}}(Y|X) - \log P_{\text{ILM}}(Y)
\label{eq:ilm}
\end{equation}

The HAT factorization makes it mathematically more stable to then integrate an E2E model with an external LM, without needing additional coverage penalties:
\begin{equation}
\centering
Y^* = \arg \max_Y \log P_{\text{E2E}}(Y|X) -
\lambda \log P_{\text{ILM}}(Y) + \gamma \log P_{\text{ELM}}(Y)
\label{eq:hat}
\end{equation}
Here, $\lambda$ and $\gamma$ are the weights on the ILM and ELM, respectively.

==> 4_related.tex <==


\section{Related Work}
\label{sec:related}

\TS{i wonder if this related work is better in the intro?}
\WW{Ehsan \& Rohit}

\RP{Relevant papers:}
Weng et al.~\cite{WengYuCuiEtAl20minimum}: One of the first papers to use MWER with RNN-T. Use transformer/TDNN-based RNN-T models, and optimize the MWER criterion over (on-the-fly) decoded N-best lists. If I understand correctly, only uses the best alignment paths. Paper also discusses shallow fusion, though they have a somewhat complicated normalization process to account for blanks. 

Guo et al.~\cite{GuoTiwariDroppoEtAl20Efficient}: MWER training of RNN-T using periodically generated lattices (i.e., not on-the-fly). No LM during MWER training. Experiment with LM rescoring for eval only. Unlike~\cite{WengYuCuiEtAl20minimum}, sums over all alignment paths during the loss computation.

Lu et al.~\cite{LuMengKandaEtAl20Minimum} MWER training specifically for HAT models. Do not train with the LM, but apply the LM with shallow fusion during inference. Show that MWER and shallow fusion gains are complementary.

\textbf{Most related work} Meng et al.~\cite{MengWuKandaEtAl21minimum} propose to optimize HAT models with LM/ILM weights during MWER training. During inference, the training weights work well. Probably need to discuss this paper early, and discuss how the current work differs.

\RP{We can also add general discriminative training papers in the context of hybrid ASR. Let me know if you'd like me to add some.}

